A Survey of Collection Methods and Cross-Data Set Comparison of Android Unlock Patterns

Android's graphical password unlock remains one of the most widely used schemes for phone unlock authentication, and it is has been studied extensively in the last decade since its launch. We have learned that users' choice of patterns mimics the poor password choices in other systems, such as PIN or text-based passwords. A wide variety of analysis and data collections methods was used to reach these conclusions, but what is missing from the literature is a systemized comparison of the related work in this space that compares both the methodology and the results. In this paper, we take a detailed accounting of the different methods applied to data collection and analysis for Android unlock patterns. We do so in two dimensions. First we systemize prior work into a detailed taxonomy of collection methods, and in the second dimension, we perform a detailed analysis of 9 different data sets collected using different methods. While this study focuses singularly on the collection methods and comparisons of the Android pattern unlock scheme, we believe that many of the findings generalize to other graphical password schemes, unlock authentication technology, and other knowledge-based authentication schemes.

==> compare.tex <==
\section{Comparing Available Data Sets}

\subsection{Most Common Patterns and Segments}

\subsubsection{Common Patterns and Shapes}

\subsubsection{Common Segments}

\subsection{Statistical Properties and Strength}

\subsubsection{Visual Features}

\subsubsection{Strength Metrics}


%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> locking.tex <==
\section{Studies on Locking Preferences}

\cite{egelman2014readytolock}

\cite{harbach2014sa}

\cite{vanbruggem2013modifying}

\cite{harbach2016anatomy}

\cite{harbach2016keep}

\cite{vonZezschwitz2013wild} 

%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> modifications.tex <==
\section{Proposed Modifications and Advancements}

\cite{DeLuca2014nowyousee} Now you see me now you don't

\cite{de2013back} Back of device authentication

\cite{kwon2014tinylock} tiny lock

\cite{von2013making} smudge safe


%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> mse.tex <==
%stating this here

\tablemse

The most basic analysis one can perform to compare datasets is to look at the
most commonly used patterns. One can visualize the most frequent patterns (such
a visual is provided in the appendix, Figure~\ref{fig:freqpatterns}), and a
casual observations provides some intuition regarding the frequency of common
shapes and sizes, as noted in prior work and we do not provide a detailed
analysis here. However, we wish to measure the similarity between the datasets,
which can be done using a pairwise of {\em Mean Square Error (MSE)}.  

The idea is that one can view the distribution of patterns as a probability
density function, as an estimator for likelihood those patterns appear in another
dataset. More frequent patterns would have higher probabilities of appearing

r distribution, and take the difference between these distribution
in frequencies as a measure of similarity between the datasets.

In the below computation, we consider vector $p$ and $q$ containing the
normalized probability of appearance for each possible pattern as computed based
on the frequency of occurrence within the dataset. The difference between the
two datasets is then computed as
\[
\operatorname{MSE}(p,q) = \frac{1}{|\text{patterns}|} \sum_{ x\in\text{patterns} }  \left( p[x]-q[x] \right)^2
\]
where $p[x]$ and $q[x]$ retrieve the normalized probability for pattern $x$ in
the dataset $p$ or $q$, respectively. The number of patterns in a 3x3 space is
389,112. If the pattern is not present in the dataset, $p[x]=0$. We note that
this similarity metric does not take into account differences in the sizes of
the datasets where $p$ may have more unique patterns than $q$. However, these
differences in unique patterns tend to happen at the long tail of the
probability density function and should have limited effect. Additionally, we do
not use statistical comparison tests here as MSE already provides a grounded
pair-wise comparison in a fixed range. 

The results are shown in Table~\ref{tab:mse} (note that all results are
$\times 10^{-8}$). We find that most datasets are similar to each other, with
LDR-banking and ZeBoDLAH being most similar in terms of the frequency of
patterns. The UDWH-def showed the most differences, as we might expect given the
methodology, but is most similar to the other defensive dataset,
ABK-MP-adv-def.



While comparing frequency distributions of complete data is informative, we can
also compare the frequencies of subsets of patterns, such as a trigram. A
trigram is a connection of three  contact points that could occur along
any part of a valid pattern. Using the same MSE comparison technique described
previously, except considering the total number of trigrams possible (488), we
can observe more similarities between these datasets in
Table~\ref{tab:mse_gram}. 

% The 20 most common trigrams across all datasets can be
% found in Figure~\ref{fig:trigrams}.\reminder{add this figure}.

Observing these results, again, many datasets are similar to each
other. Interestingly, the distributional similarity of the trigrams for the
defensive datasets is very striking and different than other datasets, as well
as the comparison between LDR-banking and ABK-MP-self as compared to other data
sets. These two datasets, are collected in similar manners and suggest that
they may be capturing similar incentives from the users with respect to the
shape of the patterns. The ZEBOdLAH dataset also has interesting properties,
showing the most similarity to the defensive datasets, despite not using an
adversarial methodology, but also showing similarity with ABK-MP-self.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> old_analysis.tex <==
\section{Methods of Analyzing Collected Datasets}

\reminder{AJA: We may be able to remove this section since we do further analysis below}
As there are different methods of collecting patterns, there are also
different analysis methods. These methods have also adapted over time
with increased complexity as the space has matured. The application of
this classification can be found in Tables~\ref{tab:collected-data}
and~\ref{tab:collected-data-alternative}; the terms can be found in
Table~\ref{tab:terms-analyze}.


\subsection{Visual Features}
The most direct and intuitive method of analyzing the data set is
based on visual features of the patterns. A classic example of a
visual feature is the length of the pattern, i.e., the number of
contact points used, but the stroke length, number of turns,
knight-moves, crosses, non-adjacencies, and shifted-ness of the
patterns have also been common metrics
(see~\cite{aviv2014understanding,song2015meteres} for further
definitions of these terms).

In ZEBOdLAH visual similarities was the focus of the analysis. The
researchers demonstrated that many patterns are rotations, flips, and
inversion of other patterns in the dataset (also observed in ABK-MP-*)
and can lead to decrease security. Based on this observation the
researchers in~\cite{zezchwitz2016onquant} changed the background
image or emphasized different starting points for the pattern to
encourage participants to select different patterns.

\subsection{Physical Attacks}
Another avenue for measuring the data set is the susceptibility of the
collected pattern to physical attacks which either require an attacker
to be proximate to the device or rely on the physical nature of
entering a pattern. Perhaps seminal to this space is the smudge
attack~\cite{aviv2010smudge} which is based on observing oily-residues on the
touchscreen surface that persist following pattern entry, but shoulder
surfing~\cite{von2015easy} and sensor based
attacks~\cite{aviv2012practicality} also fit into this category. Of
the large collected datasets, only ATOY conducted an analysis of
physical attack analysis on the data, particularly focused on smudge
attacks.

\subsection{Pattern Meters}
One method commonly employed to encourage users to select stronger
passwords is to use a password meter. The idea being that as the user
increases the complexity of their password, typically measured in the
form of length, number of upper-case, lower-case, special symbols,
etc., a colored metered increases to demonstrate the increase in
complexity. This can ``gamify'' the process of selecting a pattern and
inform the user when they have increased complexity sufficiently for
security or to meet the requirements of a password policy.

Both the SWZ and SCOKH datasets were collected in reference to pattern
meters where participants were randomly assigned to treatments where
some generated patterns using the meter and some generated patterns
without the meter~\cite{sun2014dissecting,song2015meteres}. Similarly,
SGSMA-EPSM incorporated the meter into the pattern lines as the user
enters the authentication~\cite{siadati2015fortifying}, as opposed to
having the meter external to the entry process.

%RK 12-13-2016 - There is a clause missing here

The methods
for the meters' metric calculation is often based on visual feature
calculations, e.g., how long the pattern is, rather than an
information theoretic measures, e.g., guessability, which can be
problematic in squaring the meter output to strength
measures~\cite{heidt2016refining}. However, there is some evidence
that introducing a meter does affect behavior and could lead to
increased security during pattern selection under guessability
strength metrics~\cite{song2015meteres}.

\subsection{Recall Rates}
Another important aspect of analysis is the participants ability to
recall and use the pattern. This is particularly important in studies
where incentives for generating patterns are used, e.g., adversarial
setting, and it may be the case that the patterns generated are not a
pattern that participant actually uses. Analyzing the recall rate, can
the participate recall the pattern after some sort of distraction
task, may indicate if the pattern is usable. 

Recall was used in both the UDWH-* and ABK-MP-adv-* studies to asses
the adversarial settings~\cite{aviv2015bigger,uellenbeck}. This was
particularly relevant for the altered patterns as these are not used
in the wild. A measurement of the recall rate can inform the
researchers if the alterations are realistic in comparison to the
classical pattern settings.


\subsection{Demographic Analysis}
While all the datasets report demographic breakdowns of the
participants, it is also possible to measure the if demographics play
a role in other measurements as a primary analysis technique, e.g.,
location and handedness. Two datasets applied this approach in detail:
ABK-MP-self looked at a number of demographic factors, including age,
location, and handedness as part of further
analysis~\cite{aviv2016analyzing}; and, the LDR data set investigated
similar demographic factors in detail, including hand
size~\cite{loge2016user}.

\subsection{Guessability/Entropy}

Perhaps the most grounded method for analyzing patterns is based on
their guessing strength~\cite{kelley2012guess,bonneau2012science}; how
many guesses does it take to crack the pattern? This technique is
common in text-based passwords where protection from offline attacks
are the focus of much of the strength considerations. Typically the
strength is reported in terms of entropy as an estimation of the
randomness of the patterns the user selection, which can also be
interpreted as an estimate on the number of guesses needed to crack a
password.

For patterns, as a lack of real data is not available, researchers
must first develop a guessing method based on some sample data. The
current best known techniques are based on probabilistic Markov
models that estimate the likelihood of a pattern trained on some
sample set~\cite{uellenbeck, aviv2015bigger}. Using the guesser, {\em
  partial guessing entropy}~\cite{bonneau2012science} is the preferred
method which measures a slightly different guessing estimation: the
number of guesses to crack some percentage of the data set? Partial
guessing entropy has been used in analyzing the ABK-MP-*, UDWH-* and
SCOKH data sets.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> survey.tex <==
%% \section{Survey of Collected Datasets}
%% \tableterms{}

%% In this section, we will present an overview of the relevant work on
%% collecting Android unlock patterns. Of most interest to this survey
%% paper is the methods used during that data collection and how those
%% methods have evolved over time to provide a better perspective on user
%% choice of Android unlock patterns. To do so, we will provide a
%% taxonomy of methods and organize the prior work into this taxonomy,
%% but first, we will highlight some of the challenges associated with
%% this problem space.




%% \subsection{Problems with collecting data for research on (graphical)
%%   passwords}

%% \begin{itemize}
%% \item Obtaining data for research on uer authentication is notoriously
%%   hard
%% \item Conflicting interests of collecting reliable data and ethical
%%   considerations
%% \item ...
%% \end{itemize}




%% A range of data collection methods have been adopted by researchers
%% when investigating the usable security of unlock patterns. Examples
%% include the use of online surveys to better understand user habits
%% when setting a pattern lock and their perceptions regarding what
%% constitutes a secure patterns~\cite{andriotis2013pilot}, alongside
%% questions to identify factors that may influence the strength of the
%% chosen patterns, such as gender, background in IT or IT security,
%% handedness etc.~\cite{loge2016user}.  These factors have been
%% correlated with patterns selected to better understand the behaviors
%% made by mobile users, with a view to offering more targeted password
%% advice for users.

%% The Web has been used to gather a large amount of information
%% regarding pattern choices via online surveys. Crowdsourcing platforms
%% such as MTurk have been used by a range of researchers with studies
%% conducted on the user's personal mobile device
%% (e.g.~\cite{von2015easy},~\cite{aviv2015bigger})). This has the
%% advantage of enabling researchers to conduct studies with multiple
%% users simultaneously.  Similarly, apps have been developed for use on
%% a wide range of mobile devices~\cite{song2015meteres}.  These could
%% be used to monitor behavioral changes in multiple usage scenarios over
%% time.

%% Online studies may rely on self-reporting (e.g. security experience,
%% hand size~\cite{loge2016user}, patterns~\cite{aviv2015bigger}),
%% which can pose challenges if users report incomplete or inaccurate
%% data. To ensure honesty among participants, researchers have conducted
%% attention tests, where the pattern (or statistics about their pattern)
%% should be entered twice, once at the beginning and once towards the
%% end of the study~\cite{aviv2015bigger}.  Aviv et al. presented
%% truth-based questions, along with giving participants the chance to
%% opt out of submitting their pattern if they were not comfortable
%% sharing it.

%% In terms of studies to examine physical attacks, researchers have
%% focused their efforts on recreating events which may occur in real
%% life.  Examples for local include camera, microscope and thermal
%% imaging attacks to examine the impact of the trail left when using the
%% finger on a mobile screen~\cite{andriotis2013pilot}. Researchers have
%% examined the impact of guessing attacks.  Examples include the study
%% by Aviv et al.~\cite{aviv2015bigger}, where participants were asked
%% to generate offensive and defensive patterns.  The adversarial
%% methodology was also used by Uellenbeck et
%% al.~\cite{uellenbeck2013quantifying}, encouraging users to create
%% patterns which they believe others will use (and thus would probably
%% use themselves)~\cite{aviv2015bigger}.

%% Other studies have focused on user's playing the role of victim, while
%% other participants play the role of shoulder surfers
%% (e.g.~\cite{song2015meteres}).  To improve on levels of ecological
%% validity, studies have been conducted "in the wild" to better
%% understand the behaviors users make when performing daily tasks
%% (e.g.~\cite{song2015meteres}). While lab-based studies
%% (e.g.~\cite{sun2014dissecting}) offer the benefits of more control
%% over distracters, researchers have suggested that care should be taken
%% in design of all types of study to ensure that exposure to trials does
%% not cause users to adapt their behavior~\cite{von2015easy}.  The
%% researchers have suggested that repeated measure designs are
%% unfeasible whenever behavior changes need to be observed.


%% Metrics used for evaluating pattern strength include pattern
%% length~\cite{andriotis2013pilot, song2015meteres}, directional
%% changes in patterns~\cite{andriotis2013pilot}, rotations,
%% translations, mirroring and inversions ~\cite{von2015easy}, ratio of
%% non-repeated segments and number of intersecting
%% points~\cite{song2015meteres}, positioning of starting and/or ending
%% points\cite{andriotis2013pilot}, ~\cite{von2015easy}, among others.
%% Passwords have been gathered through the device itself (termed:
%% on-device) (e.g. ~\cite{sun2014dissecting}) or through using pen and
%% paper approaches~\cite{aviv2015bigger}, the latter limiting the time factor
%% associated with setting up hardware for studies.  Various modeling
%% approaches have been adopted to identify pattern strength.  Examples
%% include the use of Markov Models to estimate the probabilities of
%% patterns ~\cite{loge2016user}, ~\cite{uellenbeck2013quantifying},
%% greedy clustering to group similar patterns ~\cite{von2015easy}.

%% Findings from studies have culminated in guidance to support graphical
%% password choice, and the design of graphical password meters
%% (e.g. ~\cite{sun2014dissecting,song2015meteres}.  Alternative patterns
%% have also been proposed by ~\cite{uellenbeck2013quantifying} better
%% support users when selecting passwords.

%% \subsection{Overview of Prior Published Work for Classical Patterns}

%% In this subsection, we will overview the key published studies that
%% performed data collection of Android unlock patterns. A summary of
%% these patterns and the data collection methods, dataset size, and
%% brief description is summarized in Tables~\ref{tab:collected-data}
%% and~\ref{tab:collected-data-alternative}. Below, we attempt to place these
%% works into context with each other and the trajectory of research in
%% this space.

%% One of the earliest attempts to measure user generated patterns was
%% from Andriotis et. al~\cite{andriotis2013pilot} where data from 144
%% participants were collected using an online, local, web-based
%% survey. Participants were asked to generate one ``secure'' and one
%% ``easy'' pattern and answer questions regarding their perceived
%% threats to those patterns. While the recruitment population was mostly
%% male and mostly young (as is typical from university hosted studies),
%% these early findings suggested that there exists issues with the
%% diversity of patterns that users select.

%% For example, Androitis et. al reported pattern lengths on average of
%% 6.64 with standard deviation of 1.92 for the ``secure'' patterns. This
%% result is common in later collected datasets. Additionally, an
%% overwelming number of participants selected patterns that start in the
%% top left and terminate towards the bottom right. Common bi-, tri-, and
%% quad-grams also match other published work.

%% A challenge with this study's methodology, as compared to later work,
%% is that incentives for participants to select realistic patterns that
%% they may actually use is not clearly defined with the procedures. As a
%% result, it could be the case that this early study may not well
%% represent the set of actually used patterns by users on their own
%% devices.

%% Following studies attempted to increase the realism of the incentive
%% structure by building in adversarial dynamics into the data collection
%% methods. Most notably, Uellenbeck et. al~\cite{uellenbeck} was the
%% first published data set to collect data on device using an adversary
%% based incentive. Following, Aviv et. al~\cite{aviv2015bigger} used a
%% similar methodology to perform their collection, except using
%% pen-and-paper, where participants literally draw patterns on paper
%% connecting contact points with a pen approximating the device
%% interaction .

%% The basics of the adversarial method requires a participant to provide
%% one or more, so called, defensive pattern which is selected with the
%% incentive that other participant should not be able to guess the
%% pattern(s). Participants also select some number of offensive patterns
%% to guess others' defensive pattern. Participants that can guess
%% another's pattern or selected a defensive pattern that was not guessed
%% receive an award.

%% The dataset collected by Uellebeck et. al targeted recruitment in a
%% cafeteria and had participants select patterns locally, on-device and
%% were rewarded with a ``treat'' if either incentives were met,
%% selecting a non-guessed defensive pattern or guessing another's
%% offensive pattern. In total 113 individuals participating generating
%% 106 valid defensive patterns and 573 offensive patterns (5 guesses
%% each).

%% Aviv et. al adopted the adversarial method during data collection, but
%% modified it to work with pen-and-paper rather than on
%% device. Additionally, rather than target general individuals in a
%% public setting, the data recruitment occurred in focused
%% groups. Within each group, participants selected 3 defensive patterns
%% and 10 offensive patterns; treats were provided if incentives were
%% met. In total, 38 individuals participated generating 114 valid
%% defensive patterns and 380 valid offensive patterns.

%% As these two data sets are available to the authors, we have conducted
%% a baseline comparison. The results are very consistent, \reminder{with
%%   pattern lengths of XXX and other properties.}. Additionally, Aviv
%% et. al in follow work~\cite{aviv2016analyzing} conducted a study
%% comparing pen-and-paper results with on-device results finding very
%% small and negligible differences.

%% What is still unclear in these studies is if the adversarial method
%% meets the expectations of real world, used-every-day patterns. It does
%% provide incentives related to security and unauthorized access, but it
%% may be the case that the defensive nature of the experiment over
%% estimates the real-world patterns individuals would choose. There is
%% some evidence that this is the case within the study by Uellenbeck and
%% Aviv et. al where the entropy scores for guess ability show significant
%% differences between offensive and defensive pattern strength. The
%% defensive patterns, particularly for the Uellenbeck study, are much
%% harder to guess. The authors note that it is likely that the offensive
%% patterns---the patterns that participants believe that others have
%% chosen rather than the one they choose themselves---are actually more
%% representative of the reality of user patterns on devices.


%% As a check on that hypothesis, Aviv et. al~\cite{aviv2015bigger}
%% conducted a second survey online using Amazon Mechanical Turk which
%% asked user to self-report the patterns they actually use on their own
%% devices. The survey allowed for participants to opt-out by providing
%% statistics, e.g., the length and starting point, rather then a
%% pattern, and it also required participants to complete the survey on
%% an their own Android device. As it was a self-reported study, there is
%% limitations in that participants may misrepresent their choice in
%% pattern or simply generate a random pattern during the survey;
%% attention tests were used to aleviate some of those concerns within
%% the study protocol. In total, 757 participants responded to the
%% survey, with 440 providing self-reported patterns as part of the
%% dataset.

%% In follow up, Aviv et. al~\cite{aviv2016analyzing} conducted a
%% methodological study comparing the self-reported dataset and the
%% pen-and-paper dataset along a many dimensions, including visual
%% features and guessability/strength. They found that the offensive
%% dataset (the patterns used to guessed others defensive patterns) had
%% properties most similar to that of the self-reported patterns. This,
%% again, suggests that these forms of data collection are getting closer
%% to the true user set of patterns on real devices. 


%% \reminder{I'm not particularly liking the structure of this
%%   section. It's too long and it needs to better match the taxonomy
%%   that we are introducing. Need to keep thinking about it --AJA}

%\figalternates{}
    
%\subsection{Overview of Prior Published work for Altered Patterns}

%\reminder{Cite Uellenbeck and 4x4 patterns --- maybe tinylock and some other ones}


%% \subsection{Classifying collection-methods}
%% There are several dimensions on which we can classify the collection
%% methods used to collect data in previous experiments.  
%% %
%% The first dimension considers the \emph{scenario} for collecting data.
%% \begin{itemize}
%% \item \emph{self-reported data}: The simplest setting for an
%%   experiment is asking the user for his/a pattern.  

%%   The experiment can \emph{ask for real patterns} of te user, but this
%%   is problematic from an ethical point of view and must at least offer
%%   the possibility to skip this step without penalty.  (And even then
%%   it is unclear if users report correctly; even worse, we conjecture
%%   that security aware people will more often \emph{not} report their
%%   real pattern, so we risk a bias in the data towards weaker
%%   patterns.)

%%   The experiment can obtain \emph{confirmation} of the pattern, i.e.,
%%   requiring second input of the same pattern.  This closely resembles
%%   the real pattern setup in Android and is very much preferred, as
%%   without confirmation participants may just enter random patterns
%%   (that they likely cannot reproduce) in an attempt to short-cut the
%%   study.

%%   One central concern with this methodology is that (i) if no
%%   confirmation is needed then participants can be tempted to enter a
%%   random pattern, and (ii) if confirmation is required then
%%   participants may choose a pattern which is very easy to type, as
%%   there is no incentive to choose a strong pattern.  (Whether people
%%   feel an incentive to choose a strong pattern during normal operation
%%   of an authnetication scheme is a different question.)

%% \item data collected in an \emph{adversarial design}: In order to
%%   give participats some incentive to choose strong patterns Uellenbeck
%%   et al.~\cite{uellenbeck} used an ``adversarial design, where
%%   a user chooses patterns and knows that they will subsequently be
%%   attacked, and being attacked successfully means only getting partial
%%   reward.

%%   Data collected in this model results in two subsets:
%%   % 
%%   The \emph{defensive set} which is the patterns chosen by the
%%   participants to ``defend'' their account.
%%   % 
%%   The \emph{offensive set} which are the patterns chosen to attack the
%%   other's users accounts.  
%%   % 
%%   We will mark those subsets by the suffixes ``-def'' and ``-off''
%%   wheen necessary.  


%% \item \emph{real data}: A third form is real data leaked from some
%%   service and available to researchers.  For text passwords, several
%%   such leaks are available and frequently used in research.  For
%%   Android Unlock Patterns (and graphical schemes in general) no such
%%   leak is known to the authors, and much more unlikely to occur as
%%   patterns are used in practice solely for device nulock and stored
%%   locally, i.e., a large-scale leak is quite unlikely.

%%   Using leaked lists of authentication secrets rises ethical
%%   questions, but the consensus seems to be that data that is publicly
%%   available anyway can be used for research purposes (with the
%%   ultimate goal of increasing the user's security), provided that
%%   certain safety meausres are used: do not distribute the data any
%%   further, publish aggregated results only and no individual
%%   passwords, ... \todo{}
  
%% \end{itemize}


%% \noindent
%% A second dimension considers where users are participating in the
%% study.
%% \begin{itemize}
%% \item \emph{online (remote) data collection}: A common and cheap
%%   method is remotely, typically recruited by crowdsourcing (such as
%%   Mechanical Turk), email lists, or social media.  
%%   % 
%%   Advantages are that typically one can more easily reach larger and
%%   more diverse participants, and they participate in the study in a
%%   well-known and familiar setting, which is hoped to introduce less
%%   bias than in-lab studies.  The main disadvantages are having little
%%   control over participants and only bottom-line data, only little
%%   process data.

%% \item \emph{local data collection}: A middle-ground between remote and
%%   inßlab data collection is local (comparable to ``Hallway testing''),
%%   where participants are selected randomly from people passing by, in
%%   a relatively natural (out-of-lab) situation, but still under the
%%   supervision of the experimentor.
%%   % 
%%   It may help to eliminate biases introduced by the in-lab setting.

%% \item \emph{in-lab data collection}: Studies performed in-lab give the
%%   researcher most control over participants and let us (to a certain
%%   extent) observe if they participate honestly.  However, there is
%%   common expectation that the obviously artificial setting biases
%%   participants responses.

%% \end{itemize}

%% \noindent
%% A third dimension is on what type of device data is collected.
%% \begin{itemize}
%% \item \emph{on device}: This means that data is collected on a device
%%   identical or very similar to the device normally used for inputting
%%   the pattern (and that the provided interface is identical or very
%%   similar).  For Android Unlock Patterns this typically means a mobile
%%   device, either the user's or a frequent model, with a very similar
%%   interface.

%% \item \emph{pen-and-paper}: Here data is colelcted on paper, usually
%%   on a pre-drawn grid closely resembling the original scheme.  The
%%   different user interface (pen isntead of finger, i.e., better
%%   visibility of the screen, usually better control of the tip etc.)
%%   could be expected to bias the data collection, however, previous
%%   work~\cite{} has indicated that the expected bias is small.\todo{}
%% \end{itemize}



%% Cite \cite{fahl-13-ecological-validity}



%% \subsection{Data collected for the ``classical'' Android Unlock Patterns}

%% The first large-scale collection of Android Pattern was published by
%% Uellenbeck et al.~\cite{uellenbeck} in 2013.  They collected data from
%% 113 participants (and 366 more for variations of the scheme, see
%% below).  They used an adversarial design, and a local on-device
%% colelction of data.  Specifically they recruited participants when
%% entering the university's mensa, and enforced a recall of the
%% collected patterns after at least 20 minutes\todo{}.  (In the meantime the
%% patterns were ``under attack''.)
%% %
%% They collected 1 defensive pattern and 5 offensive patterns per
%% participant; 106 defensive patterns were successfully recalled\todo{}
%% and 573 offensive patterns were collected \todo{this number doesn't
%%   make sense!}

%% \cite{aviv2015bigger} 


%% \cite{aviv2016analyzing} 


%% Loge et al.~\cite{loge2016user} collected patterns with the goal to
%% understand the effect of personal characteristics on pattern strength.
%% They collected data from 802 participants, in a fictious scenario for
%% protecting a fictious bank account, online shopping, and device
%% unlock.  They used an online study using the participant's own device.
%% Patterns were confirmed directly after entering them.


%% \cite{xxxsong} they collected patterns, tested a strength meter ???




%% Based on the findings of the first study (on the original Android
%% Unlock Pattern scheme, Uellenbeck et al.~\cite{uellenbeck} also
%% collected data for alternative patterns.  The setup was identical to
%% above.  They considered four variants, that are shown in
%% Figure~\ref{fig:alternatives}; one avoiding the most frequent starting
%% point upper-left, one in addition adding two more points in a fourth
%% row, one in a circular arrangement with a center node, and one in a
%% random arrangement.


%% \cite{aviv2015bigger} Guessability, self-report, adversarial collection









%% \section{Comparing the datasets}


%% \subsection{Individual guessing strength}


%% \subsection{Cross-training}


%% \subsection{Tri-gram frequencies}

%% \subsection{...}

%% \subsection{Discussion}







%% \section{Further papers on strength of Android Lock Patterns}
%% \todo{Where do we move these papers? Related work?}

%% \subsection{Measuring strength}

%% \cite{song2015meteres} \cite{sun2014dissecting}  \cite{heidt2016refining} Meters

%% \cite{andriotis2014complexity} Complexity measures



%% \subsection{Side channels and observations}

%% \cite{aviv2010smudge} Smudge Attacks

%% \cite{aviv2012practicality} Sensor Attacks

%% \cite{vonZezschwitz2015easy} \cite{schaub2012surfing} Tracability/Shoulder surfing



%% \subsection{Others}


%% \cite{aviv2014understanding} Perceptions

%% \cite{andriotis2013pilot} Pilot Study, hard and easy






%%% Local Variables:
%%% TeX-master: "main"
%%% End:

